Multi-shot Pedestrian Re-identification via Sequential Decision Making

Multi-shot pedestrian re-identification problem is at the core of surveillance video analysis. It matches two tracks of pedestrians from different cameras. In contrary to existing works that aggregate single frames features by time series model such as recurrent neural network, in this paper, we propose an interpretable reinforcement learning based approach to this problem. Particularly, we train an agent to verify a pair of images at each time. The agent could choose to output the result (same or different) or request another pair of images to verify (unsure). By this way, our model implicitly learns the difficulty of image pairs, and postpone the decision when the model does not accumulate enough evidence. Moreover, by adjusting the reward for unsure action, we can easily trade off between speed and accuracy. In three open benchmarks, our method are competitive with the state-of-the-art methods while only using 3% to 6% images. These promising results demonstrate that our method is favorable in both efficiency and performance.

==> Makefile <==
TARGET=paper

all: 
	pdflatex $(TARGET).tex
	#detex $(TARGET).tex | grep -v '^$$' > $(TARGET).txt
	bibtex $(TARGET)
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex
	rm -f $(TARGET).synctex $(TARGET).aux $(TARGET).log $(TARGET).bbl $(TARGET).blg $(TARGET).brf $(TARGET).txt $(TARGET).out

clean:
	rm -f $(TARGET).synctex $(TARGET).aux $(TARGET).pdf $(TARGET).log $(TARGET).bbl $(TARGET).blg $(TARGET).brf $(TARGET).txt $(TARGET).out
	rm -f *.log
	find . -name '*.eps' -exec rm -v {} \; 

show: all
	evince $(TARGET).pdf

